ByteCover: Cover Song Identification via Multi-Loss Training

We present in this paper ByteCover, which is a new feature learning method for cover song identification (CSI). ByteCover is built based on the classical ResNet model, and two major improvements are designed to further enhance the capability of the model for CSI. In the first improvement, we introduce the integration of instance normalization (IN) and batch normalization (BN) to build IBN blocks, which are major components of our ResNet-IBN model. With the help of the IBN blocks, our CSI model can learn features that are invariant to the changes of musical attributes such as key, tempo, timbre and genre, while preserving the version information. In the second improvement, we employ the BNNeck method to allow a multi-loss training and encourage our method to jointly optimize a classification loss and a triplet loss, and by this means, the inter-class discrimination and intra-class compactness of cover songs, can be ensured at the same time. A set of experiments demonstrated the effectiveness and efficiency of ByteCover on multiple datasets, and in the Da-TACOS dataset, ByteCover outperformed the best competitive system by 20.9\%.

==> 1_intro_bak.tex <==

\section{Introduction}
\label{sec:intro}


Cover song identification (CSI) is the task of retrieving the cover versions of the query track in a music database, which can be applied in music license management, music clustering, retrieval, and recommendation. Due to its potential applications, it has long attracted lots of researchers.

In the past decade or so, the MIR community has focused on feature engineering and the design of postprocessing strategies.   
The researcher designed various handcrafted features for encoding melodic, harmonic, or timbre information guiding by music theory \cite{marolt2006mid, kurth2008efficient}. 
Moreover, the postprocessing strategies of these methods yield transposition, tempo, timing, or structure-invariance \cite{serra2009cross, ellis2007identifying}.  These invariances encourage the CSI methods to generalize better on large and diversified music database.

Deep learning-based methods \cite{yu2020learning,doras2019cover,yesiler2020accurate,yesiler2020less} have achieved state-of-the-art performance for automatic cover song identification (CSI) in recent years. Examples include the CQTNet \cite{yu2020learning}, a convolutional neural networks(CNNs)-based model which takes the Constant-Q transform (CQT) representation of audio as input. 
The model is trained to learn a surrogate classification task to classify which version group the training sample belongs to. At the retrieval stage,  the output of the network's penultimate layer is considered a version embedding, and the similarities can be estimated with a cosine distance metric in the embedding space.

Several up-to-date works shared a similar pipeline with the CQTNet, while the input representation can also be dominant melody \cite{doras2019cover}, or chord-informed chroma \cite{yesiler2020accurate,yesiler2020less}.  

And the loss functions were as various as triplet loss\cite{doras2019cover,yesiler2020accurate} or Normalized Softmax loss \cite{yesiler2020less}. 

In general, the classification and metric learning based training schemes are two common methods for training a version descriptor. These feature learning-based methods learn to extract a compressed embedding from the input audio.
The lengths of these representation vectors are usually unrelated to the duration of input music. Thus we can construct an efficient and scalable CSI system with an approximate nearest neighbor search library \cite{johnson2017billion} while the similarity between covers can be measured by Euclidean distance or cosine distance metrics.
\par


%%https://openaccess.thecvf.com/content_WACV_2020/papers/Taha_Boosting_Standard_Classification_Architectures_Through_a_Ranking_Regularizer_WACV_2020_paper.pdf
The classification and metric learning based training schemes are two common methods for training the CSI model. 


However, there are still problems that limit the application of the CSI algorithms in real life,  one of which is the retrieval performance of the SoTA methods on the large music corpus is still far from perfect \cite{yu2020learning, yesiler2020accurate}. 

A key difficulty for a deep learning-based CSI model is learning to extract a distinguishable, robust, and light-weight feature from the input audio. 
In order to achieve this goal and further improve the retrieval performance of the model, we proposed the \ourname\ model on the basis of CQTNet. 

Compared with CQTNet, the Music-ReID model is equipped with the IBN module \cite{pan2018two}, suitable for extracting features with multiple invariants in an implicit manner.


In terms of model training, we used the technique of BNNeck \cite{luo2019strong} to integrate classification loss and triplet loss into the same objective function to achieve the mutual promotion of the two tasks. 

A key difference between the Music-ReID model and previous methods is that it prefers to learning a representation for CSI in a data-driven way. 
It is neither like MOVE \cite{yesiler2020accurate} to explicitly encode melody and chord information in the input through handcrafted features nor obtain transposition invariance through a manually-designed network structure like CQTNet.
\par


We also propose new data aggregation modules for embedding compression and data augmentation method in addition to the improvements made in the model structure and training strategy. In Section \ref{sec:approach}, we detail Music-ReID method and present the techniques used in our CSI system. In Section \ref{sec:exp}, we discuss the results of experiments conducted in four public cover song datasets. The results show that our method surpasses all previous SoTA CSI methods on all datasets by a notable margin. We conclude with future improvements to bring to our method.










==> 2_related.tex <==
\section{Related Works}
\subsection{Person Re-Identification}

Person re-identification aims at retrieving the most similar images to the probe image, from a large scale gallery setcaptured by camera networks \cite{tesfaye2019deep}. 


\subsection{Cover Song Identification}

Person re-identification aims at retrieving the most simi-lar images to the probe image, from a large scale gallery setcaptured by camera networks \cite{tesfaye2019deep}. 





\noindent \textbf{Metric Learning}.
Deep metric learning methods transform raw images into embedding features, then compute the feature distances as their similarities. Usually, two images of the same person are defined as a positive pair, whereas two images of different persons are a negative pair.
Triplet loss \cite{liu2017end} is motivated by the margin enforced between positive and negative pairs.
Selecting suitable samples for the training model through hard mining has been shown to be effective \cite{hermans2017defense, chen2017beyond, xiao2017margin}.
Combining softmax loss with metric learning loss to speed up the convergence is also a popular method \cite{geng2016deep}. 

==> 3_1_input.tex <==
\vspace{-1em}
\subsection{Input}
For the simplification of the overall pipeline, we use the CQT spectrogram rather than the PCP or other sophisticated features widely used in the CSI \cite{yesiler2020accurate}. 
%% 这里的PCP应在INTRO中定义
%The CQT spectrogram is extracted by \textit{Essentia} \cite{bogdanov2013essentia} for our system. 
In terms of the parameters of the CQT, the number of bins per octave is set as $12$ and Hann window is used for extraction with a hop size of $512$. Besides this, the audio is resampled to 22050 Hz before the feature extraction. \par 
Afterward, the CQT is downsampled with an averaging factor of 100 along the temporal dimension.  This size reduction of input feature improves the efficiency of the model and reduces the latency of our CSI system.  Finally, the input audio is processed to a compressed CQT spectrogram $S \in \mathbb{R}^{84 \times T}$, where the $T$ depends on on the duration of the input music.

==> 3_4_gempool.tex <==


\subsection{Generalized Pooling Module}
After the backbone network, the input audio has been processed to a 3-D embedding ${\cal X} \in \mathbb{R}^{K \times H \times W}$, where $K$ denotes the number of channels. 

To compress the feature map ${\cal X} \in \mathbb{R}^{K \times H \times W}$, to a fixed-length vector $\textbf{f}$f or 

Denote by ${\cal X}_k \in \mathbb{R}^{W \times H}$ the $k$-th feature map of ${\cal X}$, the most of the CSI model usually apply a pooling operation to produce a scalar $f$ representing ${\cal X}_k$ so that the input spectrogram can be represented by the vector ${\cal F} \in \mathbb{R}^{K}$. A fixed-length compacted representation vector is more suitable for large scale retrieval efficiently then high-dimensional 3-D embedding. 


Average pooling and max pooling are two common methods for aggregation of local feature, and the several CSI models \cite{yu2019temporal,yu2020learning} attach a the average pooling layer to the backbone network. At the scenario of pooling along the temporal and frequency axis simultaneously, the average pooling can be derived by:

%%TODO notation
\begin{equation}
{\cal F}^{(a)} = [f_1^{(a)} \ldots f_k^{(a)} \ldots f_K^{(a)}]^\top  \text{,\qquad}
f_k^{(a)} = \frac{1}{|{\cal X}_{k}|}\sum_{x\in {\cal X}_{k}}x
\label{equ:avgpooling}
\end{equation}
while for global max pooling  by
\begin{equation}
{\cal F}^{(m)} = [f_1^{(m)} \ldots f_k^{(m)} \ldots f_K^{(m)}]^\top  \text{,\qquad} f_k^{(m)} = \max_{x\in {\cal X}_{k}}~x
\label{equ:maxpooling}
\end{equation}



In this paper, we adapt generalized-mean (GeM) pooling, which unifies these two aggregation methods, while the compression results ${\cal F}^{(g)} $ can be given by 
\begin{equation}
{\cal F}^{(g)} = [f_1^{(g)} \ldots f_k^{(g)} \ldots f_K^{(g)}]^\top, f_k^{(g)} =\! \left( \frac{1}{|{\cal X}_{k}|}\sum_{x \in {\cal X}_{k}}\!x^{p} \right)^\frac{1}{p}
\label{equ:avgpooling}
\end{equation},
while the $p$ can adjust the behavior of the GeM pooling. In other words, the GeM pooling is equivalent to the average pooling when $p = 1$ and max pooling for $p \rightarrow \infty$. The $p$ is set to a trainable parameter to fully exploit the advantage of the deep learning. 
Furthermore, we split the regular GeM pooling into two independent operators. As Fig~\ref{fig:net}, two GeM pooling modules are applied on the along temporal and frequency dimension, respectively.


==> approach1.tex <==
\section{Approach}

\subsection{Problem Formulation}
% a training set
% find a function for feature extraction toward this task
\begin{figure}
	\centering
	\includegraphics[width=3.2in]{pipe.pdf}
	\caption{Training procedure and retrieval procedure.}
	\label{fig:pipe}
\end{figure}
As shown in \figref{fig:pipe}, we have a training dataset $D = \{(x_n, t_n)\}$, where $x_n$ is a recording and $t_n$ is a one-hot vector denoting to which song (or class) the recording belongs. Different versions of the same song are viewed as the samples from the same class, and different songs are regarded as the different classes. We aim to train a classification network model parameterized as $\{\theta,\lambda\}$ from $D$. As shown in \figref{fig:net}, $\theta$ is the parameter of all convolutions and FC$0$; $\lambda$ is the parameter of FC$1$; $f_\theta$ is the output of the FC$0$ layer. Then, this model could be used for cover song retrieval. More specifically, after the training, given a query $Q$ and references ${R_n}$ in the dataset, we extract latent features $f_\theta(Q),  {f_\theta(R_n)}$ which we call as music representations obtained by the network, and then we use a metric $s$ to measure the similarity between them. In the following sections, we will discuss the low-level representation used, the design of network structure and a robust trained model against key transposition and tempo change. We use lowercase for audio and uppercase for the CQT to discriminate.



\subsection{Low-level Representation}
The CQT, mapping frequency energy into musical notes, is extracted by \textit{Librosa} \cite{mcfee2015librosa} for our experiment. The audio is resampled to $22050$ Hz, the number of bins per octave is set as $12$ and Hann window is used for extraction with a hop size of $512$. Finally, a $20$-point mean down-sampling in the time direction is applied to the CQT, and the resulting feature is a sequence with a feature rate of about $2$ Hz. It could also be viewed as an $84 \times T$ matrix where $T$ depends on the duration of input audio.
%An visualization of CQT is shown in \figref{fig:cqt}, where the x-axis and y-axis represent time and frequency dimension respectively. Some segmentations displayed in the figure represent notes and their harmonic series in music. Compared to chroma feautres extensively used in CSI systems \cite{ellis2007identifyingcover,serra2008chroma}, CQT is a low-level feature as it does not involve projecting frequency components into twelve pitch classes. It remains more information and helps neural networks to learn a better representation for CSI. 

\subsection{Convolutional Neural Network for Key Transposition}
\begin{figure}
	\centering
	\includegraphics[width=3.2in]{cqt.pdf}
	\caption{Visualization of CQTs extracted from two versions of \textit{Twinkle Little Star}. Note that log operation is applied to make the visualization more remarkable.}
	\label{fig:cqt}
\end{figure}

Key transposition refers to that a collection of notes is moved up or down in pitch by a constant interval. \figref{fig:cqt} shows an example of key transposition. The readers could find the figures look very similar. If one shifts vertically, it becomes another one. However matching the figures on the original feature space (without consideration of transposition) fails to measure their similarity properly. To handle key transposition, straight-forward approaches test all possible transpositions or some potential transpositions \cite{ellis2007identifyingcover}:
\begin{equation}
  \label{equ:key}
  \max_{i} s(f(Q), f(R^{(i)}))
\end{equation}
in which $Q, R$ are CQTs extracted from query and reference respectively and $R^{(i)}$ represents shifting $R$ vertically for $i$ elements. Note that we have $R^{(0)} = R$. $f$ is a function indicating some post-processing to $Q$ and $R^{(i)}$, and $s$ represents some algorithm or metric to measure the similarity between $Q$ and $R^{(i)}$. Moreover, some researchers try to extract key-invariant representations; i.e. whatever the key is, the extracted features remain unchanged exactly or approximately \cite{bertin2012large,Seetharaman2017CoverSI,xu2018key}. They extract an intermediate feature satisfying that $f(R^{(i)}) = f(R^{(j)}), i \neq j$, and with this property, \equref{equ:key} becomes $s(f(Q), f(R))$. 


However previous methods use hand-crafted features for $??f$ \cite{martin2012blast,Seetharaman2017CoverSI}. In our approach, CNN is used to learn key-invariant representation. Visualizing CQTs as images, one may find that key-invariant representation is very related to shift-invariant representation in image classification. However, instead of recognizing objects in images, CNN is used to capture chord patterns or melodic structures from music. It could be used to learn a representation invariant to translations approximately \cite{goodfellow2016deep}, and thus \equref{equ:key} becomes $f(R^{(i)}) \approx f(R^{(j)}), i \neq j$ when using CNN ($\theta$ is the parameter of network). Still we find that this approximation work well in the experiments. Note that \cite{xu2018key} also use CNN to learn a key-invariant representation but their approach uses chroma sequences and aims at learning a recurrent-invariant feature. Our approach is more straight-forward and achieves much higher precision than theirs (see Section \ref{subsec:com}). 

However previous methods use hand-crafted features for $f$ \cite{martin2012blast,Seetharaman2017CoverSI}. In our approach, CNN is used to learn key-invariant representation. Ideally, given musical descriptor $Q \in R^{84 \times T}$, we assume that $Q$ is a relatively sparse matrix and most of the energy lies in a sub-matrix $Q_ \in R^{M \times T}$ ($M < 84$). $Q$ could be written as below:
 \begin{equation}
    \label{equ:key}
   \max_{i} s(f(Q), f(R^{(i)}))
 \end{equation}


\subsection{Network Structure}



\subsection{Training Scheme}


\subsection{Retrieval}
After the training, the network is used to extract music representations. As shown in \figref{fig:pipe}, given a query $q$ and a reference $r$, we first extract their CQT descriptors $Q$ and $R$ respectively, which are fed into the network to obtain music representations $f_\theta(Q)$ and $f_\theta(R))$, and then the similarity $s$, defined as their cosine similarity, are measured.
\begin{equation}
s(f_\theta(Q), f_\theta(R)) = \frac{f_\theta(Q)^Tf_\theta(R)}{|f_\theta(Q)||f_\theta(R)|}
\end{equation}
After computing the pair-wise similarity between the query and references in the dataset, a ranking list is returned for evaluation.

==> tables/0_table_bak.tex <==
% \begin{table}[!htbp]
\begin{table}
  \small
  \centering
  \label{tab:com}
  \begin{tabular}{cccccc}
      \toprule
      & MAP & P@10 & MR1 & Time  \\ 
      \midrule
      &\multicolumn{3}{c}{Results on \textit{Youtube350}} \\
      \hline
      SiMPle \cite{silva2016simple} & 0.591 & 0.140 & 7.91 & 18.7s \\ 
      TPPNet \cite{yu2019temporal}& 0.859 & 0.188 & 2.85 & 0.04ms \\
      CQT-Net \cite{zhesong} & 0.917 & 0.192 & 2.50 & 0.04ms \\
      MOVE~\cite{yesiler2020accurate}  & 0.888 & - & 3.00 \\ 
      \textbf{ByteCover}  & \textbf{0.932} & \textbf{0.201} & \textbf{2.14} & - \\ 
      \hline
      &\multicolumn{3}{c}{Results on \textit{Covers80}} \\
      \hline
      Qmax \cite{serra2009cross} & 0.544 & 0.061 & - &-\\
      Fusion \cite{chen2018fusing} & 0.625 & 0.071 & - & - \\
      %Ki-CNN \cite{xu2018key}& 0.506 & 0.068 & 16.4 & 0.55ms \\
      TPPNet \cite{yu2019temporal}& 0.744 & 0.086 & 6.88 & 0.06ms \\
      CQT-Net \cite{zhesong} & 0.840 & 0.091 & 3.85 & 0.06ms \\ 
      \textbf{ByteCover} \cite{zhesong} & \textbf{0.914} & \textbf{0.091} & \textbf{2.93} & - \\ 
      \hline
      &\multicolumn{3}{c}{Results on \textit{Da-TACOS}} \\
      \hline
      Qmax~\cite{serra2009cross}  & 0.365 & - & 113  \\
      2DFTM \cite{bertin2012large} & 0.275 & - & 155 & -  \\
      SiMPle\cite{silva2016simple} & 0.332 & - & 142 & - \\
      %Fusion \cite{chen2018fusing} & 0.454 & - & 177 & - \\
      MOVE \cite{yesiler2020accurate} & 0.507 & - & 40  \\
      Re-MOVE \cite{yesiler2020less} & 0.534 & - & 38  \\
      \textbf{ByteCover} & \textbf{0.722} & \textbf{0.972} & \textbf{2.76} & - \\
      \hline
      &\multicolumn{3}{c}{Results on \textit{SHS100K-TEST}} \\
      \hline
      2DFTM \cite{bertin2012large} & 0.104 & 0.113 & 415 & 13.9ms  \\
      Ki-CNN \cite{xu2018key}& 0.219 & 0.204 & 174 & 21.0ms \\ 
      TPPNet \cite{yu2019temporal} & 0.465 & 0.357 & 72.2 & 3.68ms \\
      CQT-Net \cite{zhesong} & 0.655 & 0.456 & 54.9 & 3.68ms \\ 
      \textbf{ByteCover} & \textbf{0.836} & \textbf{0.545} & \textbf{26.3} & - \\ 
      \bottomrule
  \end{tabular}
  \caption{Performance on different datasets (- indicates the results are not shown in original works).}
  \vspace{-2.5em}
  \end{table}

==> tables/2_ablation_1.tex <==
 \begin{table}[]
 \small
 \centering
  \begin{tabular}{cccccc}
        \toprule
        class & bbox & GIoU & AP %
        & \AP{S} %
        & \AP{L} \\
        \midrule
        \chk & \chk & &
        35.4 %
        & 13.7 %
        &       \textbf{56.4} \\
        \chk & & \chk &
        35.5 %
        & 16.6 %
        &       51.0 \\
        \chk & \chk & \chk &
        \textbf{37.3} %
        & \textbf{17.8} %
        &       54.3 \\
        \bottomrule
    \end{tabular}
    \end{table}
